Dynamical and Cosmological Aspects of Teleparallel and Extended Teleparallel Gravity

This thesis investigates modified teleparallel gravity models with a scalar field and teleparallel boundary terms, focusing on their cosmological implications for late-time cosmic acceleration. Teleparallel gravity, is an alternative to General Relativity, explains gravitation through torsion. The study presents the teleparallel analog of the Horndeski theory and its dynamical system approach, analyzing the newly developed $f(T,\phi)$ gravity model with two potential functions. It examines the phase space, conditions for different cosmological epochs, and the transition from early to late-time cosmic evolution. The inclusion of boundary terms, such as the teleparallel boundary term $B$ and the Gauss-Bonnet term $T_G$, enhances gravitational interactions. The modified teleparallel gravity models, such as $f(T, B)$, $f(T, T_G)$, and $f(T, B, T_G, B_G)$, are explored in terms of their stability and cosmological scenarios, successfully describing the accelerated expansion and late-time attractors. The thesis assesses the impact of a non-canonical scalar field coupled to the boundary term $B$ on the Universe's evolution, comparing findings from Hubble data and Supernovae Ia data. Overall, the analysis suggests that modified teleparallel gravity models effectively explain early to late-time cosmic acceleration, revealing the strong dynamical foundation and offering a versatile framework for addressing challenges in cosmic evolution.

==> Chapters/Chapter8.tex <==
% Chapter 8

%\chapter{Concluding Remarks and Future
%Perspectives} % Main chapter title

%\label{Chapter8} % For referencing the chapter elsewhere, use \ref{Chapter1} 

%\lhead{Chapter 8. \emph{Concluding remarks and future
%perspectives}} % This is for the header on each page - perhaps a shortened title




==> Makefile <==
# Makefile for BPHC Latex Report Class

LATEXMK=latexmk
LATEXOPT=-jobname="Thesis" -file-line-error
MAIN=main
THESIS=$(MAIN).tex
SOURCES=$(THESIS) Makefile

.PHONY: clean FORCE all

all: 	$(MAIN).pdf

cont: FORCE
	$(LATEXMK) -f -pdf -pvc $(LATEXOPT) $(THESIS)

$(thesis): FORCE
	latexmk -pdf -f $(thesis)

$(MAIN).pdf: .refresh $(SOURCES)
	$(LATEXMK) -f -pdf $(LATEXOPT) $(THESIS)

clean:
	$(LATEXMK) -c $(MAIN).tex
	find . \( -name "*.toc" -o -name "*.fdb_latexmk" \
							-o -name "*.pdfsync" \
                            -o -name "*.log" \
                            -o -name "*.fls" \
                            -o -name "*.aux" \
                            -o -name "*.bbl" \
                            -o -name "*.blg" \
                            -o -name "*.glo" \
                            -o -name "*.ist" \
                            -o -name "*.lof" \
                            -o -name "*.lot" \
                            -o -name "*.out" \
                            -o -name "*.toc" \
                            \) -print0 | xargs -0 rm -f

FORCE:
	touch .refresh
	$(MAKE) $(MAIN).pdf

.refresh:
	touch .refresh

